PADS: Policy-Adapted Sampling for Visual Similarity Learning

Learning visual similarity requires to learn relations, typically between triplets of images. Albeit triplet approaches being powerful, their computational complexity mostly limits training to only a subset of all possible training triplets. Thus, sampling strategies that decide when to use which training sample during learning are crucial. Currently, the prominent paradigm are fixed or curriculum sampling strategies that are predefined before training starts. However, the problem truly calls for a sampling process that adjusts based on the actual state of the similarity representation during training. We, therefore, employ reinforcement learning and have a teacher network adjust the sampling distribution based on the current state of the learner network, which represents visual similarity. Experiments on benchmark datasets using standard triplet-based losses show that our adaptive sampling strategy significantly outperforms fixed sampling strategies. Moreover, although our adaptive sampling is only applied on top of basic triplet-learning frameworks, we reach competitive results to state-of-the-art approaches that employ diverse additional learning signals or strong ensemble architectures. Code can be found under https://github.com/Confusezius/CVPR2020_PADS.

==> algorithm.tex <==


\begin{algorithm*}[t]
\label{alg:algorithm}
\caption{Training one epoch via \textit{PADS}}

\SetKwFunction{BackwardAndUpdate}{BackwardAndUpdate}
\SetKwFunction{Sample}{Sample}
\SetKwFunction{PPOLoss}{PPOLoss}
\SetKwFunction{Split}{Split}
\SetKwFunction{Backward}{Backward}
\SetKwFunction{GetBatch}{GetBatch}
\SetKwFunction{SampleActions}{SampleActions}
\SetKwFunction{Policy}{Policy}
\SetKwFunction{State}{State}
\SetKwFunction{ValMetrics}{ValMetrics}
\SetKwFunction{Reward}{Reward}
\SetKwFunction{Copy}{Copy}
\SetKwFunction{AdjustDistribution}{AdjustDistribution}
\SetKwInOut{Input}{input}
\SetKwInOut{Init}{initialization}
\SetKwInOut{Constants}{parameters}
\SetKwRepeat{Repeat}{repeat}{until}

\SetAlgoLined
% \Input{
%     Data $X$, Encoder $E$, CNN $f$,
%     Class Targets $Y_\alpha$, Minibatchsize $bs$, Number of Cluster $C$, 
%     Epochs before $Y_\beta$ update $T_U$, disentanglement $\gamma$
%     }\
\textbf{Input} Training data $X$, Labels $Y$, Network $\phi(.;\zeta)$, Criterion $\mathcal{L}$, Parametric Sampling Distr. $P$, learning rate $\lambda$, iterations per epoch $n_e$.

\textbf{PADS Parameters:} Reward/Evaluation metrics $\mathcal{E}$, train-val-split $\gamma$,  State composition: State metrics $\mathcal{E^*}$ + running average lengths $\mathcal{R}$, Policy composition: Size $s$ + Method $m$ + Support Resolution (i.e. num. actions) $res$ + Distr. Multiplicators $\{\alpha, \beta\}$, Support Limit $U_{lim}$, Distr. Prior $P^*$, $k$ iter. before $\pi$ update, $k^*$ iter. before $\pi_{old}$ update, policy learning rate $\lambda^*$.  
\newline

$P \leftarrow P^*$  

$(X_{tr}, Y_{tr}), (X_{val}, Y_{val}) \leftarrow \Split(X, Y, \gamma)$

$\pi \leftarrow \Policy(s, res, \alpha, \beta)$

$\pi_{old} \leftarrow \Copy(\pi)$
\newline

\For{i in $n_e/k$}{
    \For{j in $k$}{
        $X^b_{tr}, Y^b_{tr} \leftarrow$ \GetBatch{$X_{tr}$, $Y_{tr}$}
        
        $\Phi^b \leftarrow \phi(X^b_{tr})$ 
        
        $\mathcal{T}^{b} \leftarrow \Sample(P, \Phi^b, Y^b_{tr})$
        
        $l_{\phi} \leftarrow \mathcal{L}(\mathcal{T}^b)$
        
        $\phi \leftarrow \BackwardAndUpdate(l_{\phi}, \phi, \lambda)$
        }
        
    $E_i \leftarrow \mathcal{E}(X_{val}, Y_{val}, \phi)$

    $E^*_i \leftarrow \mathcal{E}^*(X_{val}, Y_{val}, \phi)$
    
    $S_i \leftarrow \State(E^*_i, \mathcal{R}, P)$
    
    \If{i$\geq$1}{
        $r \leftarrow \Reward(E_i, E_{i-1})$
        $l_\pi \leftarrow \PPOLoss(\pi, \pi_{old}, S_{i-1}, A_{i-1})$
        $\pi \leftarrow \BackwardAndUpdate(l_\pi, \pi, \lambda^*)$
    }
    
    $A_i \leftarrow \SampleActions(\pi(S_i))$
    $P \leftarrow \AdjustDistribution(P, A_i)$
    
    \If{i mod $M^{\text{old}}$ == 0}{
        $\pi_\theta^{old} \leftarrow \Copy(\pi)$
    }
}
    


%$(Optional)$ $f$, $\theta \leftarrow$ \Finetune{$X$, $T_{inter}$, $f$, $\theta$} 
\end{algorithm*}



==> tables/ablation_init_distr.tex <==
\begin{table*}
\begin{subtable}{1\textwidth}
  \centering
  \begin{tabular}{l|c|c|c|c}
    \toprule
    \textbf{Initial Distributions:} & uniform $\mathcal{U}_{[0,2.0]}$ & uniform $\mathcal{U}_{[0.1,1.4]}$ & $\mathcal{N}(0.5, 0.05)$ & peaked $\mathcal{I}_{[0.3,0.7]}$ \\
    \midrule
    Recall@1 & $63.5\pm 1.3 (65.2)$ & $64.0\pm 1.1 (65.5)$ & $64.8\pm 0.3 (65.2)$ & $\mathbf{65.4\pm 0.3 (65.7)}$ \\
    NMI      & $67.3\pm 0.9 (68.4)$ & $68.0\pm 0.8 (69.1)$ & $68.4\pm 0.4 (69.0)$ & $\mathbf{68.8\pm 0.3 (69.2)}$ \\
    \bottomrule
  \end{tabular}
\caption{Ablation study on usable initial distributions.}
\end{subtable}

\bigskip
\begin{subtable}{1\textwidth}
  \centering
  \begin{tabular}{l|c|c|c}
    \toprule
    \textbf{Distribution Intervals:} & $[0,2]$ & $[0,1.4]$ & $[0.1,2]$ \\
    \midrule
    Recall@1 & $63.9 \pm 0.6 (64.7)$ & $64.8 \pm 0.5 (65.2)$ & $65.1 \pm 1.0 \mathbf{(66.4)}$\\  
    NMI      & $67.4 \pm 0.1 (67.5)$ & $68.5 \pm 0.2 (68.8)$ & $68.4\pm 0.5 (69.1)$\\   
    \midrule
    \textbf{Distribution Intervals:} & $[0.1,1.4]$ & $[0.25,1.0]$ & $[0.5,1.4]$\\
    \midrule
    Recall@1 & $\mathbf{65.4 \pm 0.3} (65.7)$ & $64.2 \pm 0.5 (64.8)$ & $63.4 \pm 0.4 (63.7)$\\  
    NMI      & $\mathbf{68.8 \pm0.3 (69.2)}$ & $67.9 \pm 0.3 (68.2)$ & $67.0(0.4)67.5$\\       
    \bottomrule
  \end{tabular}
\caption{Ablation study on initial distribution interval.}
\end{subtable}

\bigskip
\begin{subtable}{1\textwidth}
  \centering
  \begin{tabular}{l|c|c|c|c}
    \toprule
    \textbf{Grid Resolution (No. Bins):} & $10$ & $30$ & $50$ & $100$\\
    \midrule
    Recall@1  & $62.7\pm 0.8 (63.8)$ & $\mathbf{65.4\pm 0.3 (65.7)}$ & $64.8\pm 0.4 (65.3)$ & $64.3\pm 0.5 (64.9)$\\
    NMI       & $67.2\pm 0.6 (67.8)$ & $\mathbf{68.8\pm 0.3 (69.2)}$ & $68.4\pm 0.4 (68.7)$ & $68.2\pm 0.3 (68.6)$\\     
    \bottomrule
  \end{tabular}
\caption{Support Grid Resolution on distance interval $[0.1,1.4]$.}
\end{subtable}
% \begin{subtable}{1\textwidth}
%   \centering
%   \begin{tabular}{l|c|c|c|c|c}
%     \toprule
%     \textbf{Grid Resolution (No. Bins):} & $10$ & $20$ & $30$ & $40$ & $50$\\
%     \midrule
%     Recall@1  & 62.7(0.8)63.8 & 64.2(0.3)64.6 & \textbf{65.4(0.3)65.7} & 65.1(0.4)65.6 & 64.8(0.4)65.3\\
%     NMI       & 67.2(0.6)67.8 & 68.0(0.6)68.9 & \textbf{68.8(0.3)69.2} & 68.6(0.3)69.0 & 68.4(0.4)68.7\\     
%     \bottomrule
%   \end{tabular}
% \caption{Support Grid Resolution on distance interval $[0.1,1.4]$.}
% \end{subtable}

\bigskip
\begin{subtable}{1\textwidth}
  \centering
  \begin{tabular}{l|c|c|c|c}
    \toprule
    \textbf{Validation Set:} & By Class & Per Class & By Class, reshuffled & Per Class, reshuffled \\
    \midrule
    Recall@1 & $61.7 \pm 0.6 (62.6)$ & $65.4\pm 0.3 (65.7)$ & $61.9\pm 0.8 (63.0)$ & $\mathbf{65.4\pm 0.4 (65.8)}$\\
    NMI      & $67.2 \pm 0.4 (67.7)$ & $68.8\pm 0.3 (69.2)$ & $67.0\pm 0.6 (67.8)$ & $\mathbf{69.3\pm 0.2 (69.6)}$\\    
    \bottomrule
\end{tabular}
\caption{Influence of validation set composition. Note that the reshuffle-value is taken for reshuffle frequency $\frac{1}{50\text{ epochs}}$, which we found to work best down to a frequency of $\frac{1}{100\text{ epochs}}$. Lower frequencies approach the standard setup and lose meaning. }
\end{subtable}
\caption{Various ablation studies on our proposed \textit{ANS} setup.}
\end{table*}

==> tables/eval_cars196.tex <==
\begin{table}
    \label{tab:cars}
    \setlength\tabcolsep{1.5pt}
    \centering
     \begin{tabular}{l|c|ccc|c}
        \toprule
        Approach & Dim & R@1 & R@2 & R@4  & NMI \\
        \midrule
        %LiftStruct \cite{lifted} & 512 & 48.3 & 61.1 & 71.8 & 55.1 \\
        %FacilityLoc \cite{facilitylocation} & 64 & 67.0 & 83.7 & 93.2 & - \\
        %SmartMin \cite{smartmining} & 64 & 64.7 & 76.2 & 84.2 & - \\
        %Angular\cite{angular} & 512 & 71.4 & 81.4 & 87.5& - \\
        % HDC\cite{hdc} & 384 & 73.7 & 83.2 & 89.5 & - \\
        % DAML\cite{daml} & 512 & 75.1 & 83.8 & 89.7 & 66.0 \\
        % Semihard\cite{semihard} & - & 51.5 & 63.8 & 73.5 & 53.4 \\
        % N-pairs\cite{npairs} & 64 & 71.1 & 79.7 & 86.5 & - \\
        Rank\cite{rankedlist}[Iv2] & 512 & 74.0 & 83.6 & 90.1 & 65.4 \\
        HTG\cite{htg} & - & 76.5 & 84.7 & 90.4 & - \\
        HDML\cite{hardness-aware} & 512 & 79.1 & 87.1 & 92.1 & 69.7 \\
        Margin\cite{margin} & 128 & 79.6 & 86.5 & 90.1 & 69.1 \\
        HTL\cite{htl} & 512 & 81.4 & 88.0 & 92.7  & - \\
        DVML\cite{dvml} & 512 & 82.0 & 88.4 & 93.3 & 67.6 \\
        A-BIER\cite{abier} & 512 & 82.0 & 89.0 & 93.2  & - \\
        MIC\cite{mic} & 128 & 82.6 & 89.1 & 93.2 & 68.4 \\
        D\&C\cite{Sanakoyeu_2019_CVPR} & 128 & 84.6 & 90.7 & 94.1 & \textbf{70.3}\\
        Ours (Margin\cite{margin} + \textit{ANS}) & 128 & 83.2 & 89.7 & 93.7 & 68.1 \\
        \hline
        \multicolumn{6}{l}{High Weight Extension} \\      
        \hline
        HORDE\cite{horde} [Iv1] & 512 & 81.5 & 88.5 & 92.7 & ? \\
        HORDE\cite{horde} [BN-Iv1] & 512 & 83.9 & 90.3 & 94.1 & ? \\
        \hline
        \multicolumn{6}{l}{Ensemble Methods} \\
        \hline
        %BIER\cite{bier} & 512 & 78.0 & 85.8 & 91.1& - \\
        Rank\cite{rankedlist}[Iv2] & 1536 & 82.1 & 89.3 & 93.7& 71.8 \\
        DREML\cite{dreml} & 9216 & 86.0 & 91.7 & 95.0 & 76.4 \\
        ABE\cite{abe} & 512 & 85.2 & 90.5 & 94.0 & ? \\
        \textbf{HORDE}\cite{horde} (ABE)[Iv1] & 512 & \textbf{86.4} & \textbf{92.0} & \textbf{95.3} & ? \\
        SOFT-TRIPLE\cite{softriple} [BN-Iv1] & 512 & 84.5 & 90.7 & 94.5 & 70.1\\
        %Margin(ReImp) & 256 & 81.5 & 88.1 & 92.8 & 67.4 \\
        %MIC\cite{mic} (concat) & 256 & 85.8 & 91.3 & 95.1 & \textbf{70.3} \\
        %Triplet\cite{semihard} + \textit{ANS} & 128 & ? & ? & ? & ? \\
        %MIC\cite{mic} + \textit{ANS} & 128 & ? & ? & ? & ? \\
        %MIC\cite{mic} + \textit{ANS} (concat) & 256 & ? & ? & ? & ? \\
        \bottomrule
    \end{tabular}
    \caption{Evaluation on CARS196\cite{cars196}.}% * indicates our ResNet50 implementation.}
\end{table}

==> tables/eval_cub200-2011.tex <==
\begin{table}
      \label{tab:cub}
      \setlength\tabcolsep{1.5pt}
      \centering
      \begin{tabular}{l|c|ccc|c}
        \toprule
        Approach & Dim & R@1 & R@2 & R@4 &  NMI \\
        \midrule
        %LiftStruct \cite{lifted} & 512 & 46.6 & 58.1 & 69.8 & 56.2 \\
        %FacilityLoc \cite{facilitylocation} & 64 & 48.2 & 61.4 & 71.8 & 59.2 \\
        %SmartMin \cite{smartmining} & 64 & 49.8 & 62.3 & 74.1 & - \\
        %Histogram\cite{histogram} & & 50.3 & 61.9 & 72.6  & - \\
        % BinDev\cite{bindeviance} & - & 52.8 & 64.4 & 74.7  & - \\
        DVML\cite{dvml} & 512 & 52.7 & 65.1 & 75.5 &61.4 \\
        % DAML\cite{daml} & 512 & 52.7 & 65.4 & 75.5 & 61.3 \\
        HDML\cite{hardness-aware} & 512 & 53.7 & 65.7 & 76.7 & 62.6 \\
        %Angular\cite{angular} & 512 & 54.7 & 66.3 & 76.0& 61.1 \\
        % HDC\cite{hdc} & 384 & 53.6 & 65.7 & 77.0 & - \\
        HTL\cite{htl} & 512 & 57.1 & 68.8 & 78.7 & - \\
        Rank\cite{rankedlist}[Iv2] & 512 & 57.4 & 69.7 & 79.2 & 62.6 \\
        HTG\cite{htg} & - & 59.5 & 71.8 & 81.3 & - \\
        A-BIER\cite{abier} & 512 & 57.5 & 68.7 & 78.3& - \\
        Margin\cite{margin} & 128 & 63.6 & 74.4 & 83.1 &69.0 \\
        D\&C\cite{Sanakoyeu_2019_CVPR} & 128 & 65.9 & 76.6 & 84.4 &69.6 \\
        MIC\cite{mic} & 128 & 66.1 & 76.8 & 85.6 & 69.7 \\
        Ours (Margin\cite{margin} + \textit{ANS}) & 128 & \textbf{67.2} & \textbf{77.9} & \textbf{86.0} & \textbf{70.2} \\
        \hline
        \multicolumn{6}{l}{Ensemble Methods} \\
        \hline
        %BIER\cite{bier} & 512 & 55.3 & 67.2 & 76.9 & - \\
        Rank\cite{rankedlist}[Iv2] & 1536 & 61.3 & 72.7 & 82.7 & 66.1 \\
        DREML\cite{dreml} & 9216 & 63.9 & 75.0 & 83.1 & 67.8 \\
        ABE\cite{abe} & 512 & 60.6 & 71.5 & 79.8 & ? \\
        HORDE\cite{horde} [Iv1] & 512 & 58.3 & 70.4 & 80.2 & ? \\
        HORDE\cite{horde} (ABE) [Iv1] & ? & 62.7 & 74.3 & 83.4 & ? \\
        HORDE\cite{horde} [BN-Iv1] & 512 & 66.3 & 76.7 & 84.7 & ? \\
        SOFT-TRIPLE\cite{softriple} [BN-Iv1] & 512 & 65.4 & 76.4 & 84.5 & 69.3\\
        %Margin(ReImp) & 256 & 65.2 & 75.9 & 84.5 & 68.1 \\
        %\textbf{MIC}\cite{mic} \textbf{(concat)} & 256 & \textbf{67.0} & \textbf{77.3} & \textbf{85.8} & 69.3 \\
        %Triplet\cite{semihard} + \textit{ANS} & 128 & ? & ? & ? & ? \\
        %MIC\cite{mic} + \textit{ANS} & 128 & ? & ? & ? & ? \\
        %MIC\cite{mic} + \textit{ANS} (concat) & 256 & ? & ? & ? & ? \\
        \bottomrule
      \end{tabular}
      \caption{Evaluation on CUB200-2011\cite{cub200-2011}.}% * indicates our ResNet50 implementation.}
\end{table}

==> tables/eval_sop.tex <==
\begin{table}
  \label{tab:sop}
  \setlength\tabcolsep{1.4pt}
  \centering
  \begin{tabular}{l|c|ccc|c}
    \toprule
    Approach & Dim & R@1 & R@10 & R@100 & NMI \\
    \midrule
    %Histogram\cite{histogram} & - & 63.9 & 81.7 & 92.2 &  - \\
    % BinDev\cite{bindeviance} & - & 65.5 & 82.3 & 92.3 &  -\\
    %LiftStruct \cite{lifted} & 512 & 63.0 & 80.5 & 91.7 & 87.4 \\
    %FacilityLoc \cite{facilitylocation} & 64 & 67.0 & 83.7 & 93.2 & -  \\
    % N-pairs\cite{npairs} & 512 & 67.7& 83.8 & 93.0 & 88.1 \\
    %Angular\cite{angular} & 512 & 70.9 & 85.0 & 93.5 & 88.6 \\
    % DAML\cite{daml} & 512 & 68.4 & 83.5 & 92.3 & 89.4 \\
    % HDC\cite{hdc} & 384 & 69.5 & 84.4 & 92.8 & - \\
    HDML\cite{hardness-aware} & 512 & 68.7 & 83.2 & 92.4 & 89.3 \\
    DVML\cite{dvml} & 512 & 70.2 & 85.2 & 93.8 & 90.8 \\
    BIER\cite{bier} & 512 & 72.7 & 86.5 & 94.0 & - \\
    Margin\cite{margin} & 128 & 72.7 & 86.2 & 93.8 & 90.7 \\
    A-BIER\cite{abier} & 512 & 74.2 & 86.9 & 94.0 & - \\
    HTL\cite{htl} & 512 & 74.8 & 88.3 & 94.8 &  - \\
    D\&C\cite{Sanakoyeu_2019_CVPR} & 128 & 75.9 & 88.4 & 94.9 &  90.2 \\
    Rank\cite{rankedlist}[Iv2] & 512 & 76.1 & 89.1 & 95.4 & 89.7 \\
    MIC\cite{mic} & 128 & 77.2 & 89.4 & 95.6 & 90.0 \\
    ALA\cite{ala} & 128 & 78.9 & 90.7 & \textbf{96.5} & ?\\
    Ours (Margin\cite{margin} + \textit{ANS}) & 128 & \red{(75.1)} & ? & ? & ? \\
    \hline
    \multicolumn{6}{l}{Ensemble Methods} \\
    \hline
    ABE\cite{abe} & 512 & 76.3 & 88.4 & 94.8 & ? \\
    Rank\cite{rankedlist}[Iv2] & 1536 & 79.8 & 91.3 & 96.3 & 90.4 \\
    HORDE\cite{horde}[Iv1] & ? & 72.6 & 85.9 & 93.7 & ? \\
    \textbf{HORDE}\cite{horde} (ABE)[BN-Iv1] & ? & \textbf{80.1} & \textbf{91.3} & 96.2 & ? \\
    SOFT-TRIPLE\cite{softriple} [BN-Iv1] & 512 & 78.3 & 90.3 & 95.9 & \textbf{92.0}\\
    
%    Margin(ReImp) & 256 & 76.1 & 88.1 & 94.9 & 89.5 \\
%    MIC\cite{mic} (concat) & 256 & 77.7 & 89.8 & 95.9 & 90.0 \\
%    Triplet\cite{semihard} + \textit{ANS} & 128 & ? & ? & ? & ? \\
%    MIC\cite{mic} + \textit{ANS} & 128 & ? & ? & ? & ? \\
%    MIC\cite{mic} + \textit{ANS} (concat) & 256 & ? & ? & ? & ? \\
    \bottomrule
  \end{tabular}
\caption{Evaluation on SOP\cite{lifted}.}% * indicates our ResNet50 implementation.}
\end{table}

==> tables/general_ablations.tex <==
\begin{table*}
\begin{subtable}{1\textwidth}
  \centering
  \begin{tabular}{l|l|c|c|c|c|c|c}
    \toprule
    \textbf{Setup} & Metrics & Ref. & Fix $\pi^*$  & Train $\pi^*$ & Train $P^*_{best}$ & Fix. $P^*_{best}$ & Fix $P^*_{full}$\\
    \midrule
    \multirow{2}{*}{Different Seed} & Recall@1 & \textbf{65.4} & 64.3 & 63.9 & 58.5 & 59.0 & 65.3\\
                                    & NMI      & 68.8 & 69.0 & \textbf{68.5} & 64.1 & 64.2 & 68.4\\
    \midrule
    \multirow{2}{*}{Same Seed}      & Recall@1 & 65.4 & \textbf{65.8} & 65.1 & 58.1 & 57.6 & -\\
                                    & NMI      & \textbf{68.8} & \textbf{68.8} & 68.4 & 63.5 & 63.7 & -\\    
    \bottomrule
\end{tabular}
\end{subtable}
\caption{Evaluation to adaptive nature of a learned policy. Transferred policies and distributions are taken when they were 10 updates away from reaching best validation performance, as the policy at the point of optimal validation corresponds to the subsequent worse results. Fixed and trained policy setup share very similar behaviour, denoting that a very specific policy for the initial training run was learned. In general, we found that policies transfer reasonably well, unlike specific distance distributions. Note that the transfer of the full distribution progression to the same seed recreates the same training results again.}
\end{table*}





